On the Compression of Language Models for Code: An Empirical Study on CodeBERT

Language models have proven successful across a wide range of software engineering tasks, but their significant computational costs often hinder their practical adoption. To address this challenge, researchers have begun applying various compression strategies to improve the efficiency of language models for code. These strategies aim to optimize inference latency and memory usage, though often at the cost of reduced model effectiveness. However, there is still a significant gap in understanding how these strategies influence the efficiency and effectiveness of language models for code. Here, we empirically investigate the impact of three well-known compression strategies -- knowledge distillation, quantization, and pruning -- across three different classes of software engineering tasks: vulnerability detection, code summarization, and code search. Our findings reveal that the impact of these strategies varies greatly depending on the task and the specific compression method employed. Practitioners and researchers can use these insights to make informed decisions when selecting the most appropriate compression strategy, balancing both efficiency and effectiveness based on their specific needs.

==> commands.tex <==
\usepackage{tikz,pifont}
\usepackage{amsfonts,amsmath}
\usepackage{hyperref}
\usepackage{xspace}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{enumitem}

\makeatletter
\let\MYcaption\@makecaption
\makeatother

\usepackage[font=footnotesize]{subcaption}

\makeatletter
\let\@makecaption\MYcaption
\makeatother


\newcommand{\nb}[2]{
	\fbox{\bfseries\sffamily\scriptsize#1}
	{\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
}
\newcommand\giord[1]{\textcolor{blue}{\nb{Giordano}{#1}}}
\newcommand\luca[1]{\textcolor{red}{\nb{Luca}{#1}}}
\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}

%Research Questions
\newcommand{\rqone}{How do compression strategies impact the efficiency and effectiveness of models fine-tuned for vulnerability detection?\xspace}
\newcommand{\rqtwo}{How do compression strategies impact the efficiency and effectiveness of models fine-tuned for code summarization?\xspace}
\newcommand{\rqthree}{How do compression strategies impact the efficiency and effectiveness of models fine-tuned for code search?\xspace}


\newtcolorbox{rqanswer}{
    colback=gray!25, % Light gray background
    colframe=black, % Border color
    enhanced,
    boxrule=0mm,
    frame hidden,
    left=1mm, % Space on the left of the text
    top=1mm, bottom=1mm, right=1mm, % Small margins
    borderline west={0.8mm}{0mm}{gray!80!black}, % Thick gray border on the left
    sharp corners, % Fully squared corners for the box
    fontupper=\small % Smaller text
}

% \newtcolorbox{shadedbox}[1]{
% title={#1},
% fonttitle=\small\bfseries,
% title filled,
% enhanced jigsaw,
% colback=white,
% boxrule=0.80pt,
% left=0.3em,
% right=0.3em,
% top=0.1em,
% bottom=0.05em
% }



==> tables/code_search_acc.tex <==
\begin{table}[tb]
    \centering
    \caption{Effectiveness of compressed code models on code search.}
    \label{tab:code_search_acc}
    \begin{tabular}{l|ccc}
\toprule
\textbf{Compression Method} & \textbf{MRR} & \textbf{MRR@1} & \textbf{MRR@5} \\
\midrule
\midrule
None & 0.329 & 0.242 & 0.310 \\
\midrule
\midrule
Know. Distil. & -52.4\% & -57.7\% & -54.3\% \\
\midrule
Pruning (0.2) & -3.2\% & -3.4\% & -3.4\% \\
Pruning (0.4) & -52.1\% & -57.3\% & -54.3\% \\
Pruning (0.6) & \underline{-99.6\%} & \underline{-99.9\%} & \underline{-99.8\%} \\
\midrule
Quantization (float8) & -0.2\% & \textbf{0.0\%} & -0.3\% \\
Quantization (int8) & \textbf{0.0\%} & -0.1\% & \textbf{+0.1\%} \\
Quantization (int4) & -6.3\% & -7.6\% & -6.7\% \\
\bottomrule
\end{tabular}
\end{table}

==> tables/code_search_eff.tex <==
\begin{table*}[tb]
    \centering
    \caption{RQ3: Inference time, model size and effectivenes of compressed models on code search.}
    \label{tab:code_search_time}
    \begin{tabular}{l|cc|c|ccc}
        \toprule
        \textbf{Compression} & \multicolumn{2}{c|}{\textbf{Inference Time}} & \textbf{Model Size} & \multicolumn{3}{c}{\textbf{Effectiveness}}\\
        \textbf{Method} & \textbf{CPU} & \textbf{GPU} & & \textbf{MRR} & \textbf{MRR@1} & \textbf{MRR@5} \\
        \midrule
        \midrule
        None & 6.047 (sec) & 0.010 (sec) & 499 (MB) & 0.329 & 0.242 & 0.310 \\
        \midrule
        \midrule
        Know. Distil. & \textbf{-84.7\% $\pm$ 0.7\%} & \textbf{-29.2\% $\pm$ 0.5\%} & -48.7\% & -52.4\% & -57.7\% & -54.3\% \\
        \midrule
        Pruning (0.2) & +5.5\% $\pm$ 1.0\% & +11.1\% $\pm$ 0.7\% & \underline{0.0\%} & -3.2\% & -3.4\% & -3.4\% \\
        Pruning (0.4) & +16.1\% $\pm$ 2.2\% & +6.4\% $\pm$ 1.4\% & \underline{0.0\%} & -52.1\% & -57.3\% & -54.3\% \\
        Pruning (0.6) & +3.1\% $\pm$ 3.5\%$^*$ & +19.8\% $\pm$ 3.3\% & \underline{0.0\%} & \underline{-99.6\%} & \underline{-99.9\%} & \underline{-99.8\%} \\
        \midrule
        Quantization (float8) & +34.2\% $\pm$ 2.9\% & +113.2\% $\pm$ 1.8\% & -51.4\% & -0.2\% & \textbf{0.0\%} & -0.3\% \\
        Quantization (int8) & +42.2\% $\pm$ 3.8\% & +105.9\% $\pm$ 1.1\% & -51.4\% & \textbf{0.0\%} & -0.1\% & \textbf{+0.1\%} \\
        Quantization (int4) & \underline{+61.8\% $\pm$ 4.8\%} & \underline{+209.6\% $\pm$ 2.0\%} & \textbf{-59.3\%} & -6.3\% & -7.6\% & -6.7\% \\
        \bottomrule
    \end{tabular}
\end{table*}

==> tables/defect_pred_acc.tex <==
\begin{table}[tb]
\caption{Effectiveness of compressed code models on vulnerability detection.}
\label{tab:defect_pred_acc}
\centering
\begin{tabular}{l|ccc}
\toprule
\textbf{Compression Method} & \textbf{Accuracy} & \textbf{F1} & \textbf{MCC} \\
\midrule
\midrule
None & 0.630 & 0.541 & 0.247 \\
\midrule
\midrule
Know. Distil. & -2.2\% & \textbf{+3.1\%} & -10.1\% \\
\midrule
Pruning (0.2) & -4.4\% & -41.0\% & -11.3\% \\
Pruning (0.4) & \underline{-7.3\%} & \underline{-61.0\%} & \underline{-20.6\%} \\
Pruning (0.6) & -5.9\% & -49.2\% & -18.2\% \\
\midrule
Quantization (float8) & \textbf{0.0\%} & -1.1\% & \textbf{+0.4\%} \\
Quantization (int8) & -0.5\% & -0.9\% & -2.4\% \\
Quantization (int4) & -1.6\% & -4.4\% & -8.5\% \\
\bottomrule
\end{tabular}
\end{table}

==> tables/defect_pred_time_size.tex <==
\begin{table*}[tb]
\caption{RQ1: Inference time, model size and effectiveness of compressed code models on vulnerability detection.}
\label{tab:defect_pred_time_size}
\centering
\begin{tabular}{l|c|c|c|c|c|c}
\toprule
\textbf{Compression} & \multicolumn{3}{c|}{\textbf{Efficiency}}  & \multicolumn{3}{c}{\textbf{Effectiveness}}\\
\textbf{Method} & \textbf{CPU Inference Time} & \textbf{GPU Inference Time} & \textbf{Model Size}   & \textbf{Accuracy} & \textbf{F1} & \textbf{MCC} \\
\midrule
\midrule
None & 15.902 (sec) & 0.011 (sec) & 499 (MB) & 0.630 & 0.541 & 0.247 \\
\midrule
\midrule
Know. Distil. & -39.8\% $\pm$ 2.7\% & \textbf{-47.7\% $\pm$ 0.6\%} & -48.8\% & -2.2\% & \textbf{+3.1\%} & -10.1\% \\
\midrule
Pruning (0.2) & +15.5\% $\pm$ 6.0\% & +9.1\% $\pm$ 2.0\% & \underline{0.0\%} & -4.4\% & -41.0\% & -11.3\% \\
Pruning (0.4) & +18.8\% $\pm$ 7.2\% & +6.2\% $\pm$ 1.7\% & \underline{0.0\%} & \underline{-7.3\%} & \underline{-61.0\%} & \underline{-20.6\%} \\
Pruning (0.6) & \textbf{-67.9\% $\pm$ 1.4\%} & +7.3\% $\pm$ 1.6\% & \underline{0.0\%} & -5.9\% & -49.2\% & -18.2\% \\
\midrule
Quantization (float8) & +41.9\% $\pm$ 16.3\% & +98.3\% $\pm$ 3.2\% & -51.4\% & \textbf{0.0\%} & -1.1\% & \textbf{+0.4\%} \\
Quantization (int8) & +102.2\% $\pm$ 14.4\% & +107.4\% $\pm$ 5.1\% & -51.4\% & -0.5\% & -0.9\% & -2.4\% \\
Quantization (int4) & \underline{+133.5\% $\pm$ 26.3\%} & \underline{+201.6\% $\pm$ 4.8\%} & \textbf{-59.3\%} & -1.6\% & -4.4\% & -8.5\% \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/summarization_acc.tex <==
\begin{table}[tb]
\caption{Effectiveness of compressed code models on Code Summarization.}
\label{tab:code_summ_acc}
\centering
\begin{tabular}{l|ccc}
\toprule
\textbf{Compression Method} & \textbf{Bleu} & \textbf{BERTScore} & \textbf{SIDE} \\
\midrule
\midrule
None & 18.791 & 0.888 & 0.871 \\
\midrule
\midrule
Know. Distil. & -42.3\% & -6.1\% & -70.6\% \\
\midrule
Pruning (0.2) & -4.3\% & -0.1\% & \textbf{+0.4\%} \\
Pruning (0.4) & -66.6\% & -17.7\% & -42.4\% \\
Pruning (0.6) & \underline{-93.4\%} & \underline{-58.4\%} & \underline{-93.0\%} \\
\midrule
Quantization (float8) & \textbf{+0.4\%} & \textbf{0.0\%} & +0.1\% \\
Quantization (int8) & -0.3\% & \textbf{0.0\%} & +0.0\% \\
Quantization (int4) & -2.0\% & -0.1\% & +0.2\% \\
\bottomrule
\end{tabular}
\end{table}

==> tables/summarization_time_size.tex <==
\begin{table*}[ht!]
    \centering
    \caption{RQ2: Inference time, model size and effectiveness of compressed code models on code summarization.}
    \label{tab:summ_time_size}
    \begin{tabular}{l|cc|c|ccc}
        \toprule
        \textbf{Compression} & \multicolumn{2}{c|}{\textbf{ Inference Time }} & \textbf{Model Size} & \multicolumn{3}{c}{\textbf{Effectiveness}} \\
        \textbf{Method}& \textbf{CPU} & \textbf{GPU} &  & \textbf{Bleu} & \textbf{BERTScore} & \textbf{SIDE} \\
        \midrule
        \midrule
        None & 157.369 (sec) & 23.692 (sec) & 707 (MB) & 18.791 & 0.888 & 0.871 \\
        \midrule
        \midrule
        Know. Distil. & -39.8\% $\pm$ 7.8\% & \textbf{-2.2\% $\pm$ 4.9\%}$^*$ & -33.0\% & -42.3\% & -6.1\% & -70.6\% \\
        \midrule
        Pruning (0.2) & \textbf{-45.3\% $\pm$ 4.9\%} & +9.8\% $\pm$ 1.9\% & \underline{0.0\%} & -4.3\% & -0.1\% & \textbf{+0.4\%} \\
        Pruning (0.4) & +24.7\% $\pm$ 19.8\% & +121.9\% $\pm$ 13.1\% & \underline{0.0\%} & -66.6\% & -17.7\% & -42.4\% \\
        Pruning (0.6) & \underline{+183.5\% $\pm$ 41.9\%} & \underline{+419.3\% $\pm$ 29.5\%} & \underline{0.0\%}  & \underline{-93.4\%} & \underline{-58.4\%} & \underline{-93.0\%} \\
        \midrule
        Quantization (float8) & -20.3\% $\pm$ 7.9\% & +14.0\% $\pm$ 2.2\% & -42.0\% & \textbf{+0.4\%} & \textbf{0.0\%} & +0.1\% \\
        Quantization (int8) & -27.2\% $\pm$ 6.7\% & +6.2\% $\pm$ 2.3\% & -42.0\% & -0.3\% & \textbf{0.0\%} & +0.0\% \\
        Quantization (int4) & -17.9\% $\pm$ 7.0\% & +29.1\% $\pm$ 2.5\% & \textbf{-51.9\%} & -2.0\% & -0.1\% & +0.2\% \\
        \bottomrule
    \end{tabular}
\end{table*}

